Distributed Resource Allocation with Binary Decisions via Newton-like Neural Network Dynamics

This paper aims to solve a distributed resource allocation problem with binary local constraints. The problem is formulated as a binary program with a cost function defined by the summation of agent costs plus a global mismatch/penalty term. We propose a modification of the Hopfield Neural Network (HNN) dynamics in order to solve this problem while incorporating a novel Newton-like weighting factor. This addition lends itself to fast avoidance of saddle points, which the gradient-like HNN is susceptible to. Turning to a multi-agent setting, we reformulate the problem and develop a distributed implementation of the Newton-like dynamics. We show that if a local solution to the distributed reformulation is obtained, it is also a local solution to the centralized problem. A main contribution of this work is to show that the probability of converging to a saddle point of an appropriately defined energy function in both the centralized and distributed settings is zero under light assumptions. Finally, we enlarge our algorithm with an annealing technique which gradually learns a feasible binary solution. Simulation results demonstrate that the proposed methods are competitive with centralized greedy and SDP relaxation approaches in terms of solution quality, while the main advantage of our approach is a significant improvement in runtime over the SDP relaxation method and the distributed quality of implementation.

==> macros-abbrev.tex <==
%% Macros for Coordination book
\newcommand{\ds}{\displaystyle}

%%%% enumerate environment containing text and with un-interrupted numbering
\newcounter{saveenum}
%% \setcounter{saveenum}{\value{enumi}}
%% \setcounter{enumi}{\value{saveenum}}

% abbreviations
\newcommand\ie{\mbox{i.e.,\xspace}}
\newcommand\eg{\mbox{e.g.,\xspace}}
\newcommand\etal{\mbox{et~al.,\xspace}}
\newcommand\etc{\mbox{etc.\@\xspace}}
\newcommand\cf{\mbox{cf.\@\xspace}}
\newcommand\resp{\mbox{resp.\@\xspace}}

\newcommand{\e}{\operatorname{e}}

%% Set definitions
\renewcommand{\natural}{{\mathbb{N}}}
\newcommand{\integer}{\ensuremath{\mathbb{Z}}}
\newcommand{\integernonnegative}{\ensuremath{\mathbb{Z}}_{\ge 0}}
\newcommand{\naturalzero}{\integernonnegative} % redundant, to remove
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\realpositive}{\ensuremath{\mathbb{R}}_{>0}}
\newcommand{\realnonnegative}{\ensuremath{\mathbb{R}}_{\ge 0}}
\newcommand{\complex}{\ensuremath{\mathbb{C}}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\SO}[1]{\mathrm{SO}(#1)}
\newcommand{\SE}[1]{\mathrm{SE}(#1)}
%% Set operations
\newcommand{\union}{\operatorname{\cup}}
\newcommand{\intersection}{\ensuremath{\operatorname{\cap}}}
\newcommand{\intersect}{\ensuremath{\operatorname{\cap}}}
\newcommand{\bigintersect}{\bigcap}

%% mathematical constructs: \setdef, \until, etc
\newcommand{\until}[1]{\{1,\dots, #1\}}
\newcommand{\subscr}[2]{#1_{\textup{#2}}}
\newcommand{\supscr}[2]{#1^{\textup{#2}}}
\newcommand{\setdef}[2]{\{#1 \; | \; #2\}}
\newcommand{\bigsetdef}[2]{\big\{#1 \; | \; #2\big\}}
\newcommand{\Bigsetdef}[2]{\Big\{#1 \; \big| \; #2\Big\}}
\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\setmap}[3]{#1: #2 \rightrightarrows #3}
\newcommand{\id}{\operatorname{id}}
\newcommand{\diag}[1]{\operatorname{diag}(#1)}
\newcommand{\setofsetvalued}[2]{\mathcal{SC}(#1,#2)}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\image}{\operatorname{image}}

%% mathematical functions
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\radius}{\operatorname{radius}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\wdist}{\operatorname{wdist}}
\newcommand{\interior}[1]{\operatorname{int}(#1)}
\newcommand{\oball}[2]{B(#1,#2)}
\newcommand{\bigoball}[2]{B\big(#1,#2\big)}
\newcommand{\Bigoball}[2]{B\Big(#1,#2\Big)}
\newcommand{\cball}[2]{\overline{B}(#1,#2)}
\newcommand{\bigcball}[2]{\overline{B}\big(#1,#2\big)}
\newcommand{\Bigcball}[2]{\overline{B}\Big(#1,#2\Big)}
\newcommand{\der}[2]{\frac{d #1}{d #2}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}

%% Symbols from Chp 2 Curves
\newcommand{\signedcurvature}{ \subscr{\kappa}{signed} }
\newcommand{\abscurvature}{ \subscr{\kappa}{abs} }
\newcommand{\radiuscurvature}{\rho}
\newcommand{\normalvector}{\operatorname{n}}
\newcommand{\innormalvector}{\operatorname{n}_{\textup{in}}}
\newcommand{\outnormalvector}{\operatorname{n}_{\textup{out}}}

%% Symbols from Chp 2 Matrix
\newcommand{\identitymatrix}[1]{I_{#1}}
\newcommand{\spectrum}{\operatorname{spec}}
\newcommand{\spectralradius}{\rho}
\newcommand{\essspectralradius}{\subscr{\rho}{ess}}

%% Symbols from Chp 2 Distributed Algorithms
\newcommand{\parts}[1]{\mathbb{P}(#1)}
\newcommand{\finite}[1]{\mathbb{F}(#1)} 
%%% make sure there are no 2^X in the final document
\newcommand{\vect}[1]{\boldsymbol{#1}}
\newcommand{\vectorones}[1][]{\vect{1}_{#1}}
\newcommand{\vectorzeros}[1][]{\vect{0}_{#1}}
\newcommand{\kernel}{\operatorname{kernel}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\proj}{\operatorname{proj}}

%% graph
\newcommand{\graph}{G}
\newcommand{\vertices}{V}
\newcommand{\edges}{E}
\newcommand{\adjmat}{A}
\newcommand{\neighbors}{\mathcal{N}}
\newcommand{\neighborsin}{\mathcal{N}^{\textup{in}}}
\newcommand{\neighborsout}{\mathcal{N}^{\textup{out}}}
\newcommand{\length}{\operatorname{length}}
\newcommand{\weight}{\operatorname{weight}}
\newcommand{\reverse}{\operatorname{rev}}
\newcommand{\TBFS}{\ensuremath{\subscr{T}{BFS}}\xspace}
\newcommand{\TDFS}{\ensuremath{\subscr{T}{DFS}}\xspace}
\newcommand{\Tshpt}{\ensuremath{\subscr{T}{shortest-paths}}\xspace}
%% \newcommand{\TMST}{\ensuremath{\subscr{T}{MST}}\xspace}
%% \newcommand{\TSP}{\ensuremath{\subscr{T}{TSP}}\xspace}
\newcommand{\algofont}[1]{\textsc{#1}}
\newcommand{\algostep}[1]{{\small\texttt{#1:}}\xspace}

%% Chp2: state machines and dynamical systems
\newcommand{\equilibria}[1]{\operatorname{Equil}(#1)}
\newcommand{\lieder}[2]{\mathcal{L}_{#1}#2}

%% Chp2: synchronous network
\newcommand{\network}[1][]{\mathcal{S}_{\textup{#1}}}
\newcommand{\Ecmm}{\subscr{E}{cmm}}

\newcommand{\alphabet}{\mathbb{A}}

%% robot and environment sensing: function, alphabet, symbol
\newcommand{\rbtsns}{\textup{rbt-sns}\xspace}
\newcommand{\rbtalphabet}{\subscr{\mathbb{A}}{rbt}}
\newcommand{\rbts}{y}

\newcommand{\envsns}{\textup{env-sns}\xspace}
\newcommand{\envalphabet}{\subscr{\mathbb{A}}{env}}
\newcommand{\envs}{\subscr{y}{env}}


\newcommand{\supind}[2]{{#1}^{[#2]}}
\newcommand{\superscr}[2]{{#1}^{\operatorname{#2}}}
\newcommand{\subind}[2]{{#1}_{[#2]}}
\newcommand{\DA}[1][]{\mathcal{D\!A}_{\textup{#1}}}
\newcommand{\timeschedule}{\integernonnegative}
\newcommand{\edtimeschedule}{\Sigma}
%\newcommand{\nll}{\mytt{null}}
\newcommand{\msg}{\textup{msg}\xspace}
\newcommand{\stf}{\textup{stf}\xspace}
\newcommand{\msgig}{\textup{msg-trig}\xspace}
\newcommand{\stftrig}{\textup{stf-trig}\xspace}
\newcommand{\msggen}{\textup{msg-gen}\xspace}
\newcommand{\msgrec}{\textup{msg-rec}\xspace}
\newcommand{\msgstandard}{\textup{msg}_{\textup{std}}}
\newcommand{\TC}{\operatorname{TC}}
\newcommand{\SC}{\operatorname{SC}}
\newcommand{\CC}{\operatorname{CC}}

%% algorithmic enviroment fixes
\newcommand{\AND}{AND\xspace}
\newcommand{\OR}{OR\xspace}
\newcommand{\return}{\textbf{return}\xspace}
\newcommand{\mycase}{\textbf{case}\xspace}
\newcommand{\mytt}[1]{\textup{\texttt{#1}}\xspace} %% mytt = my typefont text
\newcommand{\true}{\mytt{true}}
\newcommand{\false}{\mytt{false}}
\newcommand{\data}{\mytt{data}}
\newcommand{\newdata}{\mytt{new-data}}
\newcommand{\leader}{\mytt{leader}}
\newcommand{\newleader}{\mytt{new-lead}}
\newcommand{\transmit}{\mytt{transmit}}
\newcommand{\newtransmit}{\mytt{new-transmit}}
\renewcommand{\transmit}{\mytt{snd-flag}}
\renewcommand{\newtransmit}{\mytt{new-snd-flag}}
\newcommand{\search}{\mytt{search}}
\newcommand{\newsearch}{\mytt{new-search}}
\newcommand{\round}{\mytt{round}}
\newcommand{\unknown}{\mytt{unknwn}}
\newcommand{\maxuid}{\mytt{max-id}}
\newcommand{\newuid}{\mytt{new-id}} 
\newcommand{\uid}{\mytt{uid}}
\newcommand{\uuu}{\mytt{my-id}}
\newcommand{\parent}{\mytt{parent}}
\newcommand{\newparent}{\mytt{new-parent}}
\newcommand{\mydist}{\mytt{dist}}
\newcommand{\newdist}{\mytt{new-dist}}
\newcommand{\mypar}{\mytt{parent}}

%% Chp2: linear iterations
\newcommand{\TwoNorm}[1]{\|#1\|_2}
\newcommand{\bigTwoNorm}[1]{\big \|#1 \big \|_2}
\newcommand{\BigTwoNorm}[1]{\Big \|#1 \Big \|_2}
\newcommand{\PNorm}[1]{\|#1\|_p}
\newcommand{\InftyNorm}[1]{\|#1\|_{\infty}}
\newcommand{\ymaxmin}{\subscr{y}{max-min}}
\newcommand{\yerr}{\subscr{y}{err}}
\newcommand{\expfac}{\subscr{r}{exp}}

\newcommand{\tridmat}{\operatorname{Trid}}
\newcommand{\atridmat}{\operatorname{ATrid}}
\newcommand{\circmat}{\operatorname{Circ}}
\newcommand{\yave}{\subscr{y}{ave}}
\newcommand{\xave}{\subscr{x}{ave}}
\newcommand{\zave}{\subscr{z}{ave}}

\newcommand{\complexnorm}[1]{\|#1\|_\complex}
\newcommand{\Bigcomplexnorm}[1]{\Big\|#1\Big\|_\complex}
\newcommand{\norm}[2]{\|#1\|_{#2}}
\newcommand{\bignorm}[2]{\big\|#1\big\|_{#2}}
\newcommand{\Bignorm}[2]{\Big\|#1\Big\|_{#2}}
\newcommand{\Biggnorm}[2]{\Bigg\|#1\Bigg\|_{#2}}
\newcommand{\Enorm}[1]{\|#1\|_{2}}

\newcommand{\ii}{i_{\mathbb{F}}}

%% proof of number theory result
\newcommand{\mquot}{\subscr{m}{qtnt}}
\newcommand{\mremain}{\subscr{m}{rmndr}}



%% Set of matrices
\newcommand{\stoch}[1]{{\cal F}(#1)}
\newcommand{\substoch}[2]{{\cal F}_{#2}(#1)}

%% Symbols from Chp 3 Geometry
\newcommand{\PP}{\mathcal{P}}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\ov}{\overline}
\newcommand{\fti}{\operatorname{fti}}
\newcommand{\visibilityset}[2]{\operatorname{Vi}(#1;#2)}
%% \newcommand{\robustvisibilityset}[3]{\operatorname{Vi}_{#3}(#1;#2)}

%% range-limited visibility set; defined chapter 4 or 5
\newcommand{\rlvs}[2]{\subscr{\operatorname{Vi}}{disk}(#1;#2)}


%% distances
\newcommand{\distC}{\operatorname{\subscr{dist}{\texttt{c}}}}
\newcommand{\distCC}{\operatorname{\subscr{dist}{\texttt{cc}}}}

%% polytopes
\newcommand{\chull}[1]{\operatorname{co}(#1)}
\newcommand{\rchull}[2]{\operatorname{rco}_{#2}(#1)}
\renewcommand{\rchull}[2]{\operatorname{rco}(#1;#2)}
\newcommand{\co}{\operatorname{co}}

%% geometric centers
\newcommand{\ccenter}[1]{\operatorname{CC}(#1)}
\newcommand{\ccenterBig}[1]{\operatorname{CC}\!\big(#1\big)}
\newcommand{\icenter}[1]{\operatorname{IC}(#1)}
\newcommand{\cradius}[1]{\operatorname{CR}(#1)}
\newcommand{\iradius}[1]{\operatorname{IR}(#1)}
\newcommand{\area}[2]{\operatorname{A}_{#2}(#1)}
\newcommand{\centroid}[2]{\operatorname{CM}_{#2}(#1)}
\newcommand{\momentofinertia}[3]{\operatorname{J}_{#2}(#1,#3)}
\newcommand{\verticespolytope}[1]{\operatorname{Ve}(#1)}
\newcommand{\facetspolytope}[1]{\operatorname{Fa}(#1)}
\newcommand{\edgespolytope}[1]{\operatorname{Ed}(#1)}
\newcommand{\density}{\phi}
\newcommand{\Voronoi}[1]{\mathcal{V}(#1)}
\newcommand{\limVoronoi}[1]{\mathcal{V}_r(#1)}

%% proximity graphs
\newcommand{\proximitygraph}{\mathcal{G}} 
\newcommand{\edgesproximitygraph}[1]{\mathcal{E}_{#1}} 
\newcommand{\neighborsproximitygraph}{\mathcal{N}}
\newcommand{\completegraph}{\subscr{\proximitygraph}{cmplt}}
\newcommand{\rdiskgraph}{\subscr{\proximitygraph}{disk}(r)}
\newcommand{\ridiskgraph}{\subscr{\proximitygraph}{$\infty$-disk}(r)}
\newcommand{\Dgraph}{\subscr{\proximitygraph}{D}}
\newcommand{\rDgraph}[1]{\subscr{\proximitygraph}{LD}(#1)}
\newcommand{\aDgraph}{\subscr{\proximitygraph}{LD}(a)}
\newcommand{\RNgraph}{\subscr{\proximitygraph}{RN}}
\newcommand{\Ggraph}{\subscr{\proximitygraph}{G}}
\newcommand{\EMSTgraph}{\subscr{\proximitygraph}{EMST}}
\newcommand{\EMSTGgraph}[1]{\subscr{\proximitygraph}{EMST,$#1$}}
\newcommand{\Vgraph}[1]{\subscr{\proximitygraph}{vis,$#1$}}
\newcommand{\Vdiskgraph}[1]{\subscr{\proximitygraph}{vis-disk,$#1$}}
\newcommand{\ClessVdiskgraph}[1]{\subscr{\proximitygraph}{lc-vis-disk,$#1$}}
%% \newcommand{\RVgraph}{\subscr{\proximitygraph}{$\eps$-vis,Q}}
\newcommand{\LCgraph}[1]{\subscr{\proximitygraph}{lc,$#1$}}

\newcommand{\osegment}[2]{]#1,#2[}
\newcommand{\csegment}[2]{[#1,#2]}
\newcommand{\ocsegment}[2]{]#1,#2]}

%% geometric optimization
\newcommand{\HH}{\mathcal{H}}
\newcommand{\HHexp}{\mathcal{H}_{\textup{exp}}}
\newcommand{\HHdistor}{\mathcal{H}_{\textup{dist}}}
\newcommand{\HHarea}[1]{\mathcal{H}_{\textup{area},#1}}
\newcommand{\HHmixed}[1]{\mathcal{H}_{\textup{dist-area},#1}}
\newcommand{\HHworst}{\mathcal{H}_{\textup{worst}}}
\newcommand{\HHdc}{\mathcal{H}_{\textup{dc}}}
\newcommand{\HHsp}{\mathcal{H}_{\textup{sp}}}
\newcommand{\HHsum}{\mathcal{H}_\Sigma}
\newcommand{\HHmax}{\mathcal{H}_{\max}}
\newcommand{\performance}{f}
\newcommand{\coincident}{\mathcal{S}_{\textup{coinc}}}
\newcommand{\indicator}[1]{\operatorname{1}_{#1}}
\newcommand{\arc}{\operatorname{arc}}
\newcommand{\discont}[1]{\operatorname{Dscn}(#1)}

%% maybe to move into Chap 2
\newcommand{\scalarproduct}[2]{#1 \cdot #2}

%% Symbols from Chp 4 Model
\newcommand{\groupop}{\star}
\newcommand{\groupidentity}{e}
\newcommand{\so}{\mathfrak{so}}

%% Feedback communication and control + Tasks
\newcommand{\setofrobots}{\mathcal{R}}
\newcommand{\robot}{R}
\newcommand{\ctrl}{\textup{ctl}}
\newcommand{\received}[1]{\subscr{#1}{rcvd}}
\newcommand{\sensed}[1]{\subscr{#1}{snsd}}
\newcommand{\sampled}[1]{\subscr{#1}{smpld}}
\newcommand{\FCC}[1][]{\mathcal{CC}_{\textup{#1}}}
\newcommand{\ECC}[1][]{\mathcal{ECC}_{\textup{#1}}}
\newcommand{\SFC}[1][]{\mathcal{RSC}_{\textup{#1}}}
\newcommand{\task}[1][]{\mathcal{T}_{\textup{#1}}}

%% Systems Names -- polish following names: why are there 2 for each shit?
\newcommand{\disk}{disk}
\newcommand{\rdisk}{\textup{disk}}
\newcommand{\circledisk}{circle}
\newcommand{\umax}{\subscr{u}{max}}
\newcommand{\rIdisk}{$\infty$-disk}
\newcommand{\LD}{\textup{LD}}
\newcommand{\visdisk}{vis-disk}

\newcommand{\rs}[1]{\supscr{#1}{rs}}

%% FCC Names
\newcommand{\agreepursueName}{\algofont{agree \& pursue}\xspace}
\newcommand{\agreepursue}{\algofont{agree \& pursue}} %% why two?
\newcommand{\agreepursueModName}{\algofont{mod-agree \& pursue}\xspace}

\newcommand{\VicsekName}{\algofont{averaging}\xspace}
\newcommand{\circumcenter}{\algofont{crcmcntr}\xspace}
\newcommand{\nonconvexcircumcenter}{\algofont{nonconvex crcmcntr}\xspace}
\newcommand{\sensorcircumcenter}{\algofont{relative-sensing crcmcntr}\xspace}
\newcommand{\nonconvexsensorcircumcenter}{\algofont{nonconvex relative-sensing crcmcntr}\xspace}

\newcommand{\parallelcircumcenter}{\algofont{pll-crcmcntr}\xspace}
\newcommand{\parallelccenter}[1]{\operatorname{PCC}(#1)}

\newcommand{\VoronoiCentroid}{\algofont{Vrn-cntrd}\xspace}
\newcommand{\VoronoiCentroidDynamics}{\algofont{Vrn-cntrd-dynmcs}\xspace}
\newcommand{\LimitedVoronoiNormal}{\algofont{Lmtd-Vrn-nrml}\xspace}
\newcommand{\LimitedVoronoiCentroid}{\algofont{Lmtd-Vrn-cntrd}\xspace}
\newcommand{\sensorLimitedVoronoiCentroid}{\algofont{relative-sensing Lmtd-Vrn-cntrd}\xspace}
\newcommand{\RangeVoronoiCentroid}{\algofont{Rng-Vrn-cntrd}\xspace}
\newcommand{\VoronoiCircumcenter}{\algofont{Vrn-crcmcntr}\xspace}
\newcommand{\VoronoiIncenter}{\algofont{Vrn-ncntr}\xspace}

%% Task Names
\newcommand{\equidistance}{eqdstnc}

%% Sensor-based networks
\newcommand{\wrt}[2]{ \subscr{#1}{#2} }
\newcommand{\what}[2]{ \supscr{#1}{#2} }

%% Costs
\newcommand{\MCC}{\operatorname{MCC}}
\newcommand{\TCC}{\operatorname{TCC}}
\newcommand{\cc}{\operatorname{IH-MCC}}
\newcommand{\unidir}{\operatorname{unidir}}
\newcommand{\omnidir}{\operatorname{omnidir}}
\newcommand{\nonnllmsgs}{{cmm$\setminus\emptyset$}}
\newcommand{\CommCost}[1][]{\subscr{\operatorname{C}}{rnd}^{#1}}


%%% more about the agree and pursue
\newcommand{\dm}{\mytt{dir}}
\newcommand{\newdm}{\mytt{new-dir}}
\newcommand{\csym}{\mytt{c}}
\newcommand{\ccsym}{\mytt{cc}}
\newcommand{\kprop}{\subscr{k}{prop}}
\newcommand{\Hset}{H}%
\newcommand{\nHset}{n_H}%

%%% random definitions
\newcommand{\fl}[1]{\left\lfloor #1\right\rfloor}
\newcommand{\argmin}{\ensuremath{\operatorname{argmin}}}
\newcommand{\argmax}{\ensuremath{\operatorname{argmax}}}
\newcommand{\arginf}{\ensuremath{\operatorname{arginf}}}
\newcommand{\argsup}{\ensuremath{\operatorname{argsup}}}
\newcommand{\myboolean}{\ensuremath{\{\true,\false\}}} %%to erase

\newcommand{\WW}{{\mathcal{W}}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\Pc}{{\mathcal{P}}}
\newcommand{\reschedule}[3]{{#1}_{(#2,#3)}}
\newcommand{\newC}{\CommCost[]\circ\MM}
\newcommand{\Infnorm}[1]{\|#1\|_{\infty}}

%% symbols for Chp5: rendezvous

%% connectivity maintenance
\newcommand{\XConstrSet}{\mathcal{X}}
\newcommand{\XConstrSetVis}{\subscr{\mathcal{X}}{\visdisk}}
\newcommand{\XConstrSetClessVis}{\subscr{\mathcal{X}}{lc-\visdisk}}

%%\newcommand{\Dc}{\subscr{\UConstrSet}{constraint}}
%%\newcommand{\UConstrSet}{\mathcal{U}}
%%\newcommand{\UConstrSetVis}{\subscr{\mathcal{U}}{\visdisk}}

\newcommand{\rendezvous}{rndzvs}
\newcommand{\ccsalgo}{\algofont{iterated truncation}\xspace}
\newcommand{\rsccsalgo}{\algofont{relative-sensing iterated truncation}\xspace}
\newcommand{\average}{\operatorname{avrg}}
\newcommand{\vers}{\operatorname{vers}}
\newcommand{\piSpace}[1]{\pi_{#1}}


\newcommand{\maximize}{\text{maximize}}
\newcommand{\subj}{\text{subject to}}

\newcommand{\mynum}[1]{{\small\ensuremath{{\texttt{#1}}}\xspace}}

\newcommand{\EE}{\mathcal{E}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\FF}{\mathcal{F}}

%% copyright
\newcommand\reg{$^{\textrm{\tiny\textregistered}}$\xspace}

%% packages for Chp5

\usepackage{psfrag}

%% symbols for Chp 6: Deployment

\newcommand{\deployment}{dply}
\newcommand{\deploymentdistor}{distor-\deployment}
\newcommand{\deploymentarea}{area-\deployment}
\newcommand{\deploymentmixed}{distor-area-\deployment}
\newcommand{\deploymentdc}{dc-\deployment}
\newcommand{\deploymentdcwk}{dc-wk-deployment}
\newcommand{\deploymentsp}{sp-\deployment}
\newcommand{\deploymentspwk}{sp-wk-deployment}

\newcommand{\fcase}[1]{\ensuremath{(\mathbf{#1})}\xspace}
\newcommand{\Pave}{\subscr{P}{ave}}

\newcommand{\centrd}{centrd}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\incenVor}{incntr-Vor}
\newcommand{\circumVor}{crcntr- Vor}

%% symbols for Chp 7: estimation
\newcommand{\Kstf}[1]{\subscr{\supind{K}{#1}}{stf}}
\newcommand{\Kstfna}{\subscr{K}{stf}}

\newcommand{\nip}{\subscr{n}{ip}}
\newcommand{\pdistance}{\mathcal{D}_\lambda}
\newcommand{\arclengthdist}{\subscr{\mathcal{D}}{arc}}
\newcommand{\kapadistance}{\subscr{\mathcal{D}}{curvature}}

\newcommand{\nw}{\mytt{nxt}}
\newcommand{\nwrec}{\mytt{nxtrec}}
\newcommand{\curves}{\mathcal{C}}
\newcommand{\mypath}{\mytt{path}}
\newcommand{\tpath}{\mytt{t}_\mytt{path}}
\newcommand{\tangentat}{\mytt{tangentat}}
\newcommand{\cyclicbalance}{\mytt{cyclic-balance}}
\newcommand{\perpproj}{\mytt{perp-proj}}
\newcommand{\sat}{\operatorname{sat}}
\newcommand{\inclusion}{\operatorname{\iota}}

\newcommand{\eul}{\textsc{Single-Robot Estimate Update Law}\xspace}
\newcommand{\ceul}{\textsc{Cooperative Estimate Update Law}\xspace}
\newcommand{\eupl}{\textsc{Estimate Update and Balancing Law}\xspace}
\newcommand{\aupl}{\textsc{Approximate Estimate and Balancing Law}\xspace}

%% %% OLD ??
%% \newcommand{\optplace}{\mytt{opt-place}}

%% \newcommand{\lw}{\mytt{L}}
%% \newcommand{\setpath}{\operatorname{path}}
%% \newcommand{\regionest}{\mytt{\polygon}}

%% \newcommand{\timewindow}{\mytt{t}}
%% \newcommand{\prev}{\mytt{qprev}}
%% \newcommand{\apdistance}{\mytt{d}}


%% \newcommand{\forget}{\mytt{forget}}

\newcommand{\arclengthparam}{\subscr{s}{arc}}
\newcommand{\gammaarc}{\subscr{\gamma}{arc}}
% \newcommand{\arclength}{\subscr{\gamma}{arc}}
\newcommand{\gammapolar}{\subscr{\gamma}{polar}}
\newcommand{\sign}{\operatorname{sign}}

\newcommand{\Vc}{{\mathscr{V}}}
\newcommand{\Wc}{{\mathscr{W}}}
\newcommand{\Tc}{{\mathscr{T}}}
\newcommand{\Cc}{{\mathscr{C}}}
\newcommand{\Ec}{{\mathscr{E}}}
\newcommand{\DD}{{\mathcal{D}}}
\newcommand{\UU}{{\mathcal{U}}}
\newcommand{\LL}{{\mathcal{L}}}
\newcommand{\ip}{{\mytt{q}}}
\newcommand{\SeqNorm}[1]{\|#1\|_{2,\infty}}
\newcommand{\classK}{\ensuremath{\mathcal{K}}}
\newcommand{\classKinfty}{\ensuremath{\mathcal{K}_{\infty}}}
\newcommand{\classKL}{\ensuremath{\mathcal{KL}}}
\newcommand{\NearNeigh}{\text{NN}}
\newcommand{\NatNeigh}{\text{Nat}}
\newcommand{\triangular}{\text{TIN}}
\newcommand{\inverse}{\text{IDW}}
\newcommand{\localinv}{\text{LIDW}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\MSE}{\operatorname{MSE}}

\newcommand{\Tmin}{\subscr{T}{min}}
\newcommand{\ymin}{\subscr{y}{min}}
\newcommand{\xfree}{\supscr{x}{free}}
\newcommand{\xctrl}{\supscr{x}{ctrl}}

%\renewcommand{\ymaxmin}{\subscr{y}{M-m}}
\newcommand{\Aerr}{\subscr{F}{err}}
\newcommand{\cerr}{\subscr{c}{err}}
\newcommand{\Derr}{\subscr{D}{err}}
\newcommand{\Dave}{\subscr{D}{ave}}
\newcommand{\yerrtilde}{\subscr{\tilde{y}}{err}}

\setlength{\tabcolsep}{3pt}

